Operator Covariant Transform and Local Principle

We describe connections between the localization technique introduced by I. B. Simonenko and operator covariant transform produced by nilpotent Lie groups.

==> mydef.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%       $Id: mydef.tex,v 1.47 2011/03/11 19:03:34 kisilv Exp $    
%
%  File mydef.tex
%
\typeout{This is MyDef macros file}
\makeatletter
\def\ifundefined#1{\expandafter\ifx\csname#1\endcsname\relax}
\hyphenation{di-men-sio-nal}
%% Do not uncomment---does not work
%\ifundefined{tthtrue}
%  \newif\iftth
%\fi
\providecommand{\comment}[1]{}
\def\smnegskip{\mskip-0.6\thinmuskip}
\usepackage{amsfonts}
%\newlength{\curmathsize}
%
%   Objects
%
\providecommand{\algebra}[1]{\ensuremath{\mathfrak{#1}}}
\providecommand{\Heisen}[1]{{\ensuremath{\mathbb{H}^{#1}}}}
\providecommand{\hHeisen}[1]{\ensuremath{\widehat{\mathbb {H}}^{#1}}}
\providecommand{\Cliff}[2][\comment]{{\ensuremath{%
\mathcal{C}\kern-0.18em\ell(#1,#2)}}}
\providecommand{\uir}[3][0]{\ifcase #1{\rho^{#2}_{#3}}% 
\or {\breve{\rho}^{#2}_{#3}}%
\or {\tilde{\rho}^{#2}_{#3}}\fi}
%\providecommand{\Cliff}[2][\comment]{\ensuremath{\mathbf{Cl}(#1,#2)}}
\providecommand{\object}[2][\,]{\ensuremath{\mathrm{#2}#1}}
\providecommand{\Space}[3][]{\ensuremath{\mathbb{#2}^{#3}_{#1}{}}}
\providecommand{\such}{\,\mid\,}
\providecommand{\Jacobian}[1]{\ensuremath{\mathcal{J}(#1)}}
  \providecommand{\FSpace}[3][]{\ensuremath{\ifx#2l \ell_{#3}^{#1}{}\else
  #2_{#3}^{#1}{}\fi}} 
  \providecommand{\limlike}[1]{\mathop {\operator@font #1}}
  \providecommand{\loglike}[1]{\mathop {\operator@font #1}\nolimits}
\providecommand{\Quater}{\ensuremath{\mathcal{H}}}
\providecommand{\bos}{\mathcal{B}}
\ifundefined{qed}
    \DeclareMathSymbol{\qed}{0}{AMSa}{"03}
\fi
\providecommand{\SL}[1][2]{\ensuremath{\mathrm{SL}_{#1}(\Space{R}{})}}
\providecommand{\SU}[1][1,1]{\ensuremath{\mathrm{SU}(#1)}}
\providecommand{\Sp}[1][n]{\ensuremath{\mathrm{Sp}(#1)}}
%
%  Unary operations
%
\providecommand{\fourier}[1]{\ensuremath{\mathcal{F}^{#1}{}}}
\providecommand{\bra}[1]{\ensuremath{\left\langle#1\right|}}
\providecommand{\ket}[1]{\ensuremath{\left|#1\right\rangle}}
\providecommand{\Cplus}{\ensuremath{C^{+}}}
\providecommand{\Cstar}{\ensuremath{C^{*}}}
\providecommand{\onvol}{^{+}}
\providecommand{\spec}[1][]{\ensuremath{\mathbf{sp}}\,}
\providecommand{\sr}{\ensuremath{\mathbf{r}}\,}
\providecommand{\kernel}{\ensuremath{\mathbf{ker}}\,}
\providecommand{\ad}{\ensuremath{\mathbf{ad}}\,}
\providecommand{\diag}{\mathop {\operator@font diag}\nolimits}
\providecommand{\norm}[2][\relax]{\left\|#2\right\|\ifx#1\relax\else_{#1}\fi}
\providecommand{\modulus}[2][\relax]{\left| #2 \right|\ifx#1\relax\else_{#1}\fi}
\providecommand{\oper}[1]{\mathcal{#1}}
\providecommand{\rmi}{\mathrm{i}}
\providecommand{\rme}{\mathrm{e}}
\providecommand{\rmh}{\mathrm{j}}
\providecommand{\rmp}{\varepsilon}
\providecommand{\tr}{\mathop{tr}}

%
%  Binary operations%
\providecommand{\scalar}[3][\relax]{\left\langle #2,#3 
        \right\rangle\ifx#1\relax\else_{#1}\fi}
\providecommand{\intersect}[2]{\left.#1\right|_{#2}}
\providecommand{\relstack}[2]{{\mathrel {\mathop {#1}\limits _{#2}}}}
%
%
%
\providecommand{\eqref}[1]{\textup{(\ref{#1})}}
\providecommand{\eqnright}[1]{\qquad\qquad  #1}
\providecommand{\person}[1]{\textsc{#1}}
%
%  WWW commands
%
\providecommand{\href}[2]{#2}
    %\ifundefined{MR}
        \providecommand{\MR}[1]{MR\href{http://www.ams.org/mathscinet-getitem?mr=#1}{#1}}
    %\else
    %    \renewcommand{\MR}[1]{ %\textbf{MR}~
    %\href{http://www.ams.org/mathscinet-getitem?mr=#1}{#1}}
    %\fi
  \providecommand{\Zbl}[1]{Zbl\href{http://www.emis.de:80/cgi-bin/zmen/ZMATH/en/zmathf.html?first=1&maxdocs=3&type=html&an=#1&format=complete}{#1}}

\providecommand{\myeprint}[2]{E-print: \href{#1}{\texttt{#2}}}
\providecommand{\mailto}[1]{\href{mailto:#1}{\texttt{#1}}}
\providecommand{\urltt}[1]{\href{#1}{\texttt{#1}}}
\providecommand{\wiki}[2]{\href{http://en.wikipedia.org/wiki/#1}{#2}}
\providecommand{\doi}[1]{doi: \href{http://dx.doi.org/#1}{#1}}

\newif\ifhevea
\newif\ifrawhtml
%\newenvironment{rawhtml}{\ifrawhtml}{\fi}
%
\makeatother
\endinput

